Feature-Model-Guided Online Learning for Self-Adaptive Systems

A self-adaptive system can modify its own structure and behavior at runtime based on its perception of the environment, of itself and of its requirements. To develop a self-adaptive system, software developers codify knowledge about the system and its environment, as well as how adaptation actions impact on the system. However, the codified knowledge may be insufficient due to design time uncertainty, and thus a self-adaptive system may execute adaptation actions that do not have the desired effect. Online learning is an emerging approach to address design time uncertainty by employing machine learning at runtime. Online learning accumulates knowledge at runtime by, for instance, exploring not-yet executed adaptation actions. We address two specific problems with respect to online learning for self-adaptive systems. First, the number of possible adaptation actions can be very large. Existing online learning techniques randomly explore the possible adaptation actions, but this can lead to slow convergence of the learning process. Second, the possible adaptation actions can change as a result of system evolution. Existing online learning techniques are unaware of these changes and thus do not explore new adaptation actions, but explore adaptation actions that are no longer valid. We propose using feature models to give structure to the set of adaptation actions and thereby guide the exploration process during online learning. Experimental results involving four real-world systems suggest that considering the hierarchical structure of feature models may speed up convergence by 7.2% on average. Considering the differences between feature models before and after an evolution step may speed up convergence by 64.6% on average. [...]

==> sections/discussion.tex <==
We discuss current limitations of our online learning strategies.

\textbf{Feature interactions.}
As explained in Section~\ref{sec:evaluation}, our online learning strategies currently do not consider the impact of feature interactions when determining which features to explore in the evolved system.
In particular this means that old features may be explored only very late for the evolved system, even though they would lead to an effective configuration in combination with the new features in the evolved system. 
Considering such feature interactions may allow improving the evolution-aware online learning strategies.
We consider this an interesting topic for future work, which may build on existing solutions for feature interaction analysis in software product lines~\cite{ThumAKSS14,MetzgerBLP05}.

\textbf{Feature modifications.}
To address system evolution, our strategies analyze the differences in the feature models of the self-adaptive system before and after evolution.
Thereby, our strategies can determine configurations that were added or removed from the system's adaptation space.
A further possible change introduced during system evolution is the modification of a feature's implementation.
However, such a change is not visible in the feature model, and therefore our strategies are not able to consider this kind of knowledge.
Encoding this kind of knowledge such that it can be exploited during online learning thus could be a potential future direction.

\textbf{Configuration and adaptation constraints.} 
Our learning strategies are based on the assumption that switching from one valid configuration to any other valid configuration is always possible, \ie we assume that there are no technical or logical constraints on adaptation. 
On the one hand, this means we are not concerned with the technicalities of how to switch between the configurations in the running system.
This is the scope of other work, such as~\cite{ArcegaFHC16,ChenPYNZ14}, which thus may serve to address this concern.
On the other hand, we do not take into account stateful or sequential constraints on adaptation itself.
This means, in our case we can switch directly between any of the configurations in our adaptation space, without the need to go through intermediate configurations.
However, in reality, only certain paths may be permissible to reach another configuration from the current one.
As future work, we thus plan enhancing our strategies to also consider the sequence of adaptations (adaptation paths), \eg building on work such as~\cite{RamirezCMB10,Sousa_SEAMS_2017}.

\textbf{Extension to model-based adaptation.} 
In this article, we focused on rule-based adaptation.
Even though our strategies were developed for rule-based adaptation, the main ideas underlying our strategies may also be applicable for model-based adaptation.
In model-based adaptation, the aim of online learning is to learn accurate models that in turn facilitate deriving effective adaptation actions.
To this end, representative observations of the system and environment need to be collected.
As an important difference to rule-based adaptation, convergence has to be measured differently in model-based adaptation.
Here, the accuracy of the model is a prerequisite for effective adaptations.
Therefore, it is of interest how fast online learning converges on an accurate model.
We aim to further investigate online learning for model-based adaptation as part of future work.

\textbf{Extension of reinforcement learning.} 
As evident from the state of the art analysis in Section~\ref{sec:related_work}, reinforcement learning is the most widely used online learning technique for self-adaptive systems.
Our online learning strategies from Section~\ref{sec:fbased} may be used to extend existing reinforcement learning algorithms.
As an example, they may be used to augment the exploration phase of temporal-difference reinforcement learning algorithms, such as SARSA or Q-Learning~\cite{RL}.
Instead of randomly selecting the next action during exploration, our strategies may be used to better guide action selection. 
In fact, the experimental results presented above can be considered the result of employing temporal-difference reinforcement learning, in which only exploration has been performed.
In reinforcement learning terms, we set $\epsilon = 1$ for the $\epsilon$-greedy approach, which thus will choose exploration over exploitation with a probability of 1.
However, the aforementioned reinforcement learning algorithms assume that the set of actions remains constant.
Yet, during evolution the set of adaptation actions (the adaptation space) may change.
As part of future work, we thus aim to further analyze how our evolution-aware online learning strategies may be integrated with existing reinforcement learning algorithms.

\textbf{Risks and limitations of online learning.}
Despite many successful applications of online learning for self-adaptive systems (\eg see Section~\ref{sec:related_work}), online learning may not be applicable for all kinds of self-adaptive systems.
In particular, systems may operate in an environment where the effects of the trial-and-error nature of online learning may not be tolerable, because adaptation actions may harm their environment~\cite{RL}.
A typical example are safety-critical systems.
For such kinds of systems, online learning may face a too high risk as to be practically applicable.








==> sections/figure.tex <==
\begin{figure*}[htbp!]  
\centering 
  \begin{subfigure}[b]{0.4\linewidth}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Evolution step},
    ylabel={\% of explored configurations},
    xmin=0, xmax=7,
    ymin=0, ymax=90,
    xtick={0,1,2,3,4,5,6,7},
    ytick={0,10,20,30,40,50,60,70},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=6cm,height=6cm,    
    legend style={nodes={scale=0.75, transform shape}}, 
]    
    \addplot[
    dashed,
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
    (0,50)(1,50)(2,55)(3,51)(4,53)(5,52)(6,48)(7,51)
    };
    \addlegendentry{Without evolution learning}
    
    \addplot[
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
    (0,55)(1,44)(2,50)(3,33)(4,64)(5,60)(6,20)(7,9)
    };
    \addlegendentry{With learning - Random}
    
        \addplot[
    color=red,
    mark=triangle,
    ]
    coordinates {
    (0,51)(1,43)(2,47)(3,28)(4,58)(5,54)(6,13)(7,4)
    };
    \addlegendentry{With learning - IncConfdeg}

\end{axis}
\end{tikzpicture}%
    \caption{BerkeleyJ} \label{fig:Berkeley}  
  \end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Evolution step},
    ylabel={\% of explored configurations},
    xmin=0, xmax=7,
    ymin=0, ymax=90,
    xtick={0,1,2,3,4,5,6,7},
    ytick={0,10,20,30,40,50,60,70},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=6cm,height=6cm,
    legend style={nodes={scale=0.8, transform shape}}, 
]
 
\addplot[
    dashed,
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
	(0,65)(1,55)(2,57)(3,49)(4,51)(5,49)(6,50)(7,50)   
	};
    \addlegendentry{Without evolution learning}

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0,55)(1,50)(2,49)(3,24)(4,13)(5,6)(6,3)(7,51)   
    };
    \addlegendentry{With evolution learning}

\end{axis}
\end{tikzpicture}
\caption{BerkeleyC} \label{fig:BerkeleyC}  
\end{subfigure}

%% Line 2
\vspace{5mm}
  \begin{subfigure}[b]{0.4\linewidth}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Evolution step},
    ylabel={\% of explored configurations},
    xmin=0, xmax=10,
    ymin=0, ymax=80,
    xtick={0,1,2,3,4,5,6,7,8,9,10},
    ytick={0,10,20,30,40,50,60,70},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=7cm,height=5cm,    
    legend style={nodes={scale=0.8, transform shape}}, 
]
 
\addplot[
    dashed,
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
	(2,50)(3,50)(4,50)(5,53)(6,47)(7,47)(8,53)(9,53)(10,51)    
	};
    \addlegendentry{Without evolution learning}

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (2,50)(3,25)(4,13)(5,53)(6,3)(7,2)(8,1)(9,1)(10,1)    
    };
    \addlegendentry{With evolution learning}

\end{axis}
\end{tikzpicture}
\caption{LLVM} \label{fig:LLVM}  
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Evolution step},
    ylabel={\% of explored configurations},
    xmin=0, xmax=4,
    ymin=0, ymax=90,
    xtick={0,1,2,3,4},
    ytick={0,10,20,30,40,50,60,70},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=5.5cm,height=5.5cm,
    legend style={nodes={scale=0.7, transform shape}}, 
]
 
\addplot[
    dashed,
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
	(1,50)(2,51)(3,51)(4,49)
	};
    \addlegendentry{Without evolution learning}

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,52)(2,4)(3,1)(4,1) 
    };
    \addlegendentry{With evolution learning}

\end{axis}
\end{tikzpicture}
\caption{CloudRM (energy consumption)} 
\label{fig:learningCloudRM_energy} 
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Evolution step},
    ylabel={\% of explored configurations},
    xmin=0, xmax=4,
    ymin=0, ymax=90,
    xtick={0,1,2,3,4},
    ytick={0,10,20,30,40,50,60,70},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=5.5cm,height=5.5cm,    
    legend style={nodes={scale=0.7, transform shape}}, 
]    
    \addplot[
    dashed,
    color=blue,
    mark=square,
    mark options=solid,
    ]
    coordinates {
	(1,51)(2,52)(3,49)(4,51)
	};
    \addlegendentry{Without evolution learning}
    
    \addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,50)(2,4)(3,1)(4,30) 
    };
    \addlegendentry{With evolution learning}

\end{axis}
\end{tikzpicture}
\caption{CloudRM (number of migrations)} 
\label{fig:learningCloudRM_mig}
\end{subfigure}
\caption{Convergence rate for the different use cases (RQ3)}
\label{fig:comparison} 
\end{figure*}  









%\begin{figure}[!htbp]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=7,
%    ymin=0, ymax=90,
%    xtick={0,1,2,3,4,5,6,7},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=7cm,height=7.5cm,
%]    
%    \addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%    (0,50)(1,50)(2,55)(3,51)(4,53)(5,52)(6,48)(7,51)
%    };
%    \addlegendentry{Without evolution learning}
%    
%    \addplot[
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%    (0,55)(1,44)(2,50)(3,33)(4,64)(5,60)(6,20)(7,9)
%    };
%    \addlegendentry{With learning - Random}
%    
%        \addplot[
%    color=red,
%    mark=triangle,
%    ]
%    coordinates {
%    (0,51)(1,43)(2,47)(3,28)(4,58)(5,54)(6,13)(7,4)
%    };
%    \addlegendentry{With learning - IncConfdeg}
%
%\end{axis}
%\end{tikzpicture}
%\caption{BerkeleyJ - Scenario 1 (RQ3)\todo{@Clement: Figures to be updated as discussed}} 
%\label{fig:comparison1}
%\end{figure}
%
%\begin{figure}[!h]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=7,
%    ymin=0, ymax=80,
%    xtick={0,1,2,3,4,5,6,7},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=7cm,height=7.5cm,
%]
% 
%\addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%    (0,50)(1,51)(2,53)(3,55)(4,52)(5,52)(6,50)(7,50)
%    };
%    \addlegendentry{Without evolution learning}
%
%\addplot[
%    color=blue,
%    mark=square,
%    ]
%    coordinates {
%    (0,53)(1,50)(2,45)(3,35)(4,26)(5,19)(6,15)(7,13)
%    };
%    \addlegendentry{With learning - Random}
%    
%    \addplot[
%    color=red,
%    mark=triangle,
%    ]
%    coordinates {
%    (0,53)(1,50)(2,43)(3,28)(4,18)(5,10)(6,5)(7,4)
%    };
%    \addlegendentry{With learning - IncConfdeg}
%
%\end{axis}
%\end{tikzpicture}
%\caption{BerkeleyJ - Scenario 2 (RQ3)} 
%\label{fig:comparison2}
%\end{figure}
%
%\begin{figure}[!h]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=7,
%    ymin=0, ymax=90,
%    xtick={0,1,2,3,4,5,6,7},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=7cm,height=7cm,
%]
% 
%\addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%	(0,65)(1,55)(2,57)(3,49)(4,51)(5,49)(6,50)(7,50)   
%	};
%    \addlegendentry{Without evolution learning}
%
%\addplot[
%    color=blue,
%    mark=square,
%    ]
%    coordinates {
%    (0,55)(1,50)(2,49)(3,24)(4,13)(5,6)(6,3)(7,51)   
%    };
%    \addlegendentry{With evolution learning}
%
%\end{axis}
%\end{tikzpicture}
%\caption{BerkeleyC (RQ3)} 
%\label{fig:learningBerkeleyC}
%\end{figure}
%
%
%\begin{figure}[!h]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=10,
%    ymin=0, ymax=80,
%    xtick={0,1,2,3,4,5,6,7,8,9,10},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=8.5cm,height=7cm,
%]
% 
%\addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%	(2,50)(3,50)(4,50)(5,53)(6,47)(7,47)(8,53)(9,53)(10,51)    
%	};
%    \addlegendentry{Without evolution learning}
%
%\addplot[
%    color=blue,
%    mark=square,
%    ]
%    coordinates {
%    (2,50)(3,25)(4,13)(5,53)(6,3)(7,2)(8,1)(9,1)(10,1)    
%    };
%    \addlegendentry{With evolution learning}
%
%\end{axis}
%\end{tikzpicture}
%\caption{LLVM (RQ3)}
%\label{fig:learningLLVM}
%\end{figure}
%
%
%\begin{figure}[!h]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=4,
%    ymin=0, ymax=90,
%    xtick={0,1,2,3,4},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=7cm,height=7cm,
%]
% 
%\addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%	(1,50)(2,51)(3,51)(4,49)
%	};
%    \addlegendentry{Without evolution learning}
%
%\addplot[
%    color=blue,
%    mark=square,
%    ]
%    coordinates {
%    (1,52)(2,4)(3,1)(4,1) 
%    };
%    \addlegendentry{With evolution learning}
%
%\end{axis}
%\end{tikzpicture}
%\caption{CloudRM \emph{w.r.t.} energy consumption (RQ3)} 
%\label{fig:learningCloudRM_energy}
%\end{figure}
%
%\begin{figure}[!h]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Evolution step},
%    ylabel={\% of explored configurations},
%    xmin=0, xmax=4,
%    ymin=0, ymax=90,
%    xtick={0,1,2,3,4},
%    ytick={0,10,20,30,40,50,60,70},
%    legend pos=north west,
%    ymajorgrids=true,
%    grid style=dashed,
%    width=7cm,height=7cm,
%]
%
%    
%    \addplot[
%    dashed,
%    color=blue,
%    mark=square,
%    mark options=solid,
%    ]
%    coordinates {
%	(1,51)(2,52)(3,49)(4,51)
%	};
%    \addlegendentry{Without evolution learning}
%
%    
%    \addplot[
%    color=blue,
%    mark=square,
%    ]
%    coordinates {
%    (1,50)(2,4)(3,1)(4,30) 
%    };
%    \addlegendentry{With evolution learning}
%
%\end{axis}
%\end{tikzpicture}
%\caption{CloudRM \emph{w.r.t.} number of migrations (RQ3)} 
%\label{fig:learningCloudRM_mig}
%\end{figure}




==> sections/implementation.tex <==
\section{Proof of Concept}
\label{sec:poc}

As a proof of concept, this section describes an extension of reinforcement learning.
We first explain how reinforcement learning may be applied to self-adaptive systems, and then sketch how we extend reinforcement learning by incorporating our learning strategies.

\subsection{Reinforcement Learning for Self-Adaptive Systems}
\label{sec:RL}

%% CITE if needed: kulkarni2012reinforcement

\textbf{Foundations.}
As introduced in Section~\ref{sec:sota_RL}, reinforcement learning is a machine learning technique in which an agent\footnote{In the context of reinforcement learning, an \emph{agent} is any software system equipped with sensors and actuators to observe its surrounding environment and modify its behavior accordingly.} 
interacts with its environment to learn from observations which action to perform to react to a situation \todo{state??} to maximize a reward function~\cite{RL}. 
\todo{explain reward in general.}
\todo{AM will provide a more theoretical background to introduce RL; e.g., ~\cite{BarrettHD13}}

\citefig{rl} shows the main concepts underlying reinforcement learning.
At time point $i$, the agent tries an action $a_i$ and receives an immediate or delayed reward $r_i$. 
The reward indicates the agent's profit or gained utility, and is measured after the action is completed. 
Thus, the reward quantifies the success of an action in fulfilling the agent's goals and requirements.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\columnwidth]{fig/rl}
	\caption{Reinforcement Learning.}
	\label{fig:rl}
\end{figure}

An agent reacts to changes in the state of the agent's environment as follows.
Given the current state of the environment $s_i$ the agent determines an action $a_i$.
Actions may be determined by two different mechanisms: exploitation recommends the action with the highest reward, whilst exploration recommends an action (typically chosen randomly) regardless of its reward value.
Exploration, on the other hand, considers all possible actions including those never chosen before. 
Thereby, exploration prevents being stuck with sub-optimal actions.
An appropriate balance between exploitation and exploration allows the agent to learn from past experience while considering new opportunities.

\textbf{Reinforcement Learning for Self-Adaptive Systems.}
In our case, REWARD is ...?
The situation is the actual environment situation faced by the system during operation.
The action is the re-configuration of the system in order to adapt the system to the new environment (see Section~\ref{sec:FM} above).
The best-performing configuration within the new environment, i.e., the configuration that leads to the highers reward, becomes the ``rule'' for use whenever this environment is encountered~\cite{FilhoP17}.
\todo{explain and maybe illustrate this in terms of our example rules from Sec 2}



\begin{table}[!h]
\centering
\begin{tabular}{cc}
\toprule
RL concept & Self-adaptive system concept \\
\midrule
Agent & Managed element \\
Action & Adaptation (reconfiguration) \\
Reward & Satisfaction of quality requirements \\
Episode & Iteration?? \\
... & ...\\
\bottomrule
\end{tabular}
\caption{Mapping of reinforcement learning concepts to self-adaptive system concepts.}
\label{table:savings}
\end{table}


We use a simple implementation of reinforcement learning: SARSA...

** the algo could go to the section below...

\begin{algorithm}
\caption{Extended Reinforcement Learning (SARSA)}
\label{algo:random}
\begin{algorithmic}[1] %1 for numbering

\State Initialize $Q(s,a)$ arbitrarily;
\Repeat (for each episode):
  \State Initialize $s$;
	\State Choose $a$ from $s$ using policy derived from $Q$ (e.g., $\epsilon$-greedy and calling \textsc{Explore()})
	\Repeat (for each step of episode):
	  \State Take action $a$, observe $r, s'$;
		\State Choose $a'$ from $s'$ using policy derived from $Q$ (e.g., $\epsilon$-greedy and calling \textsc{Explore()})
		\State $Q(s,a) \leftarrow Q(s,a) + \alpha[r + \iota Q(s',a') - Q(s,a)]$
	  \State $s \leftarrow s'; a \leftarrow a'$;
\Until $s$ is terminal;
\Until $s$ is terminal;
\end{algorithmic}
\end{algorithm}

Algorithm is based on SARSA as presented in ~\cite{RL}.


\subsection{Extending RL with Strategies}
\label{sec:RLplus}

\todo{explain: exploration = search; exploitation = + / - sets}


\subsection{Implementation}
\label{sec:impl}

\todo{explain Java based implementation of strategies + use of any libraries used to compute valid FMs, variation degree}







